LESS: Selecting Influential Data for Targeted Instruction Tuning

Instruction tuning has unlocked powerful capabilities in large language models (LLMs), effectively using combined datasets to develop generalpurpose chatbots. However, real-world applications often require a specialized suite of skills (e.g., reasoning). The challenge lies in identifying the most relevant data from these extensive datasets to effectively develop specific capabilities, a setting we frame as targeted instruction tuning. We propose LESS, an optimizer-aware and practically efficient algorithm to effectively estimate data influences and perform Low-rank gradiEnt Similarity Search for instruction data selection. Crucially, LESS adapts existing influence formulations to work with the Adam optimizer and variable-length instruction data. LESS first constructs a highly reusable and transferable gradient datastore with low-dimensional gradient features and then selects examples based on their similarity to few-shot examples embodying a specific capability. Experiments show that training on a LESS-selected 5% of the data can often outperform training on the full dataset across diverse downstream tasks. Furthermore, the selected data is highly transferable: smaller models can be leveraged to select useful data for larger models and models from different families. Our qualitative analysis shows that our method goes beyond surface form cues to identify data that exemplifies the necessary reasoning skills for the intended downstream application.

==> sections/adam.tex <==
\section{Data Selection with Influence Functions}\label{sec:derivation}

\mz{background first, influence functions}
\mz{adam to method}
Influence functions~\citep{hampel1974influence} have traditionally been used in deep learning to trace how a particular training datapoint affects model performance on a test datapoint~\citep{koh2017understanding}.
Here, we apply influence functions to select training data.
Precise computation often requires inverting the Hessian, which is resource-intensive for LLMs, so we instead adapt the approach in~\citet{pruthi2020estimating} of using a first-order approximation of training dynamics to estimate the influence.\footnote{See~\Cref{sec:related_work} for a more detailed discussion of past works.}
The primary technical challenge to overcome, then, is that such algorithms have traditionally focused on estimating the influence when training with SGD, but LLMs are tuned with the Adam optimizer.
This section describes the first-order approximation of the influence of a training datapoint and how the approximation can be adapted to the Adam optimizer.

\paragraph{Per-Step Influence.} Consider a model $\vtheta^t$ at time step $t$ trained on the loss $\ell(\cdot;\vtheta)$.
We can write the first-order Taylor expansion of the loss on any datapoint $\vz'$ as 
	\begin{equation*}
	\resizebox{\linewidth}{!}{$
	\ell(\vz';\vtheta^{t+1}) \approx \ell(\vz';\vtheta^t) + \langle\nabla\ell(\vz';\vtheta^t), \vtheta^{t+1}-\vtheta^t\rangle $}
\end{equation*}

Assume that we are training the model with SGD with batch size $1$ and learning rate $\eta_t$.\footnote{We discuss learning rate schedules and larger batch sizes in~\Cref{sec:nuance}.}
If $\vz$ is the training data at time step $t$, we can write the SGD update as $\vtheta^{t+1} - \vtheta^t = -\eta_t \nabla\ell(\vz;\vtheta^t)$, so 
\begin{gather*}
	\resizebox{\linewidth}{!}{$
	\ell(\vz';\vtheta^{t+1}) - \ell(\vz';\vtheta^t) \approx -\eta_t \langle\nabla\ell(\vz;\vtheta^t), \nabla\ell(\vz';\vtheta^t)\rangle $}
\end{gather*}
While~\citet{pruthi2020estimating} used this insight to identify mislabeled training data, we use this insight to design a data selection strategy in the transfer learning setting. 
We can see that selecting $\vz$ to maximize $\langle\nabla\ell(\vz';\vtheta^t), \nabla\ell(\vz;\vtheta^t)\rangle$ will drive a larger decrease in the loss on the validation point $\vz'$.
\sm{I think we mention Han et al. in a footnote here}
Notably, $\vz'$ need not have any relation to the training data $\vz$, which makes this data selection strategy especially useful in the transfer learning setting.
\sm{Measure test loss and discuss how loss and generation are not necessarily related?}

\paragraph{Extension to Adam.}
The above derivation is unique to optimizing models with SGD. However, LLMs, which primarily use Transformer architectures, are typically trained using the Adam optimizer.
In this case, the model update is as follows: 
\begin{gather*}
	\vtheta^{t+1} - \vtheta^t = -\eta_t \update{\vz}{\vtheta^t} \\
	\update{\vz}{\vtheta^t} \triangleq \frac{\vm^{t+1}}{\sqrt{\vv^{t+1} + \epsilon}} \\
	\vm^{t+1} = (\beta_1\vm^t + (1-\beta_1)\grad{\vz}{\vtheta^t}) / (1-\beta_1^t) \\
	\vv^{t+1} = (\beta_2\vv^t + (1-\beta_2)\grad{\vz}{\vtheta^t}^2) / (1-\beta_2^t) 
\end{gather*}
where all vector operations are performed elementwise, with $\beta_1$ and $\beta_2$ as the exponential decay rates for the first moments $\vm$ and second moments $\vv$, respectively, and $\epsilon$ as a small constant.
We can thus write the first-order expansion for the Adam dynamics and see that we need to choose $\vz$ to maximize $\langle \grad{\vz'}{\vtheta^t}, \update{\vz}{\vtheta^t}\rangle$.

%\subsection{Additional Details}
\paragraph{Trajectory Influence.}
Measuring the gradient similarities at every training step $t$ in order to select the next datapoint is prohibitively expensive. 
If $\{t_\vz\}$ denotes the time steps where $\vz$ is trained on, then we can write the total influence of $\vz$ on $\vz'$ as $\sum_{t\in\{t_\vz\}}\eta_t\infadam(\vz, \vz')$.
Since $\vz$ is used once per epoch, it is natural to rewrite this as a summation over epochs, which yields the following definition.
\begin{definition}[Optimizer-Aware Influence]\label{def:influence}
	Suppose the model is trained for $N$ epochs, where $\bar\eta_i$ is the average learning rate in the $i$th epoch and $\vtheta_i$ is the model checkpoint after the $i$th epoch.
 %\sm{check with mengzhou, before or after $i$th epoch?}.
	We define the optimizer-aware influence of a training datapoint $\vz$ on a validation datapoint $\vz'$ as 
	\begin{gather*}
	\infadam(\vz, \vz') \triangleq \sum_{i=1}^N \bar\eta_i \langle \grad{\vz'}{\vtheta_i}, \update{\vz}{\vtheta_i}\rangle \label{eq:infadam}\\
	\infsgd(\vz, \vz') \triangleq \sum_{i=1}^N \bar\eta_i \langle \grad{\vz'}{\vtheta_i}, \grad{\vz}{\vtheta_i}\rangle \label{eq:infsgd}
	\end{gather*}
	where $\infadam$ corresponds to training with Adam and $\infsgd$ corresponds to SGD. % \mz{Do we want them both in main or SGD could go to footnote?} 
\end{definition}
Thus, we can see that measuring the influence over the entire trajectory requires training the model on at least a few of these examples, so that the gradient and optimizer update is close to what it would be during the actual training run.
In \Cref{sec:grad_features}, we describe how to perform this warmup training efficiently.  


\paragraph{Estimating $\update{\vz}{\vtheta}$.} 
The Adam weight update $\update{\vz}{\vtheta}$ relies on the $\vm$ and $\vv$ terms determined by prior training gradients.
As such, unlike SGD, including or excluding other training points changes the weight update induced by a given training point $\vz$, thereby changing the influence of $\vz$ on $\vz'$. 
This makes the data selection problem circular, since the influence of each point depends on the set of points selected.
We approximate $\vm$ and $\vv$ using the optimizer state after each epoch of the warmup training to compute $\Gamma(\vz, \cdot)$ for all $\vz$.\footnote{We compare this approach to using $\textrm{sign}(\grad{\cdot}{\vtheta})$ as an approximation for $\update{\vz}{\vtheta}$, as suggested in past theoretical works~\citep{malladi2022sdes,malladi2023kernel}. Please see~\Cref{app:adam_sgd}.}









==> sections/alg.tex <==

% \begin{figure}[t]
%     \centering
%     \begin{algorithm}
%     % \SetKwFunction{update}{UpdateWeight}
%     % \SetKwProg{sub}{Subroutine}{}{}
    
%     % \textbf{Require}: Full training data ${mathcal{D}_{\mathrm{train}}}$, a small set of target validation data ${mathcal{D}_{\mathrm{val}}}$\\
% %   \vspace{0.5em}
  
  
% %   \vspace{0.2cm}
% %   \sub{\update{$w$, $\Delta$}}{
% %     $\alpha \gets w \cdot \exp \left( \Delta \right)$ \Comment{Calculate the unnormalized weights} \\ 
% %     $w \gets \frac{\alpha}{\sum_i \alpha[i]}$ 
% %     \Return $w$ \Comment{Renormalize the data loading proportion}
% %   }
  
% %   \Return $\theta$ 
  
%   \caption{Gradient-based Data Selection} %
%   \label{alg:gradient-ds}
%   \end{algorithm}
% \end{figure}

% \begin{algorithm}
%     \caption{Gradient-based Data Selection}
%     \KwIn{A collection of training data ${\mathcal{D}_{\mathrm{train}}}$, a small set of target validation data ${\mathcal{D}_{\mathrm{val}}}$, a target datset size $k$} 
%     \KwResult{A selected subset}
%     Initialization\;
%     \While{termination condition not met}{
%         Perform some computation\;
%         Update parameters\;
%     }
%     \Return{Final result}\;
% \end{algorithm}


% \begin{algorithm}
%     \caption{Gradient-Based Data Subset Selection}
%     \KwData{Full instruction tuning dataset $\dfull$, target validation dataset $\dval$, number of epochs $N$, dimension $d$, diversity parameter $\lambda$}
%     \KwResult{Selected subset $\dsub$}
    
%     \textbf{Step 1: Initial training with LoRA}\\
%     Initialize model parameters $\vtheta$ with a pre-trained model\;
%     Train the model with LoRA on $\dfull$ for $N$ epochs, saving checkpoints at each epoch\;
    
%     \textbf{Step 2: Compute projected gradients}\\
%     Initialize $\dsub$ as an empty set\;
%     \For{each datapoint $\vz \in \dfull$}{
%         \For{each checkpoint $\vtheta_i$}{
%             Compute the projection of gradient $\projgrad{\vz}{\vtheta_i}$ using random projections\;
%         }
%     }
    
%     \textbf{Step 3: Gradient Matching}\\
%     Initialize $\hat\gD$ as an empty set\;
%     \For{each datapoint $\vz \in \dfull$}{
%         Compute the matching score for $\vz$ using \eqref{eq:match}\;
%         Add $\vz$ to $\hat\gD$ if it maximizes the matching score\;
%     }
    
%     \textbf{Step 4: Gradient Diversification}\\
%     Initialize $\dsub$ as an empty set\;
%     \While{the desired number of examples is not reached}{
%         Select the datapoint $\vz$ from $\dfull \setminus \dsub$ that maximizes $\text{matching}(\vz, \dval) + \lambda \cdot \text{diversity}(\vz, \hat\gD)$\;
%         Add $\vz$ to $\dsub$\;
%     }
    
%     \Return{$\dsub$}
% \end{algorithm}


\begin{algorithm*}
\SetKwComment{Comment}{}{}
\caption{Gradient-Based Dataset Selection}
\label{alg:subset}
\KwIn{
	Full dataset $\dfull$,
	target validation dataset $\dval$,
	desired subset size $K$,
	projected gradients $\{\projgrad{\vz}{\vtheta_i}\}\}_{i=1}^N$ for all $\vz\in\dfull$,
	candidate buffer ratio $c$
}
Construct $\texttt{M}$ to contain all $\vz\in\dfull$ in decreasing order of $\match{\vz}{\dval}$ \;
$\dsub\leftarrow\dsub\cup\{\texttt{M[0]}\}$ \;
$\texttt{M}\leftarrow\texttt{M}\setminus \{\texttt{M[0]}\}$ \;
%Add \texttt{M[0]} to $\dsub$ and delete \texttt{M[0]} from \texttt{M} \;
$\texttt{csize} = \lfloor cK\rfloor$ \;
\While{$|\dsub| \leq K$}{
    \texttt{candidates = M[:csize]} \tcp*[r]{Top candidates by matching score} 
    %Construct $\hat\gD$ by sampling $k$ examples from $\dsub$ \tcp*[r]{To efficiently compute diversity score}
    \texttt{selected} = $\texttt{argmax}_{\vz\in\texttt{candidates}} \diverse{\vz}{\dsub}$ \; 
    $\dsub\leftarrow\dsub\cup\{\texttt{selected}\}$ \;
    $\texttt{M}\leftarrow\texttt{M}\setminus \{\texttt{selected}\}$ \;
    %Add \texttt{selected} to $\dsub$ and delete \texttt{selected} from \texttt{M} \;
}
Return $\dsub$ \;
\end{algorithm*}


\iffalse
\begin{algorithm*}
    \caption{Gradient-Based Dataset Selection}
    \KwData{Full instruction tuning dataset $\dfull$, target validation dataset $\dval$, number of epochs $N$, dimension $d$, diversity parameter $\lambda$, desired subset size $K$, buffer ratio $c$, random sample number $q$}

    \KwResult{Selected subset $\dsub$}
    
    \textbf{Initialization:} Initialize $\dsub$ as an empty set
    
    \textbf{Compute the buffer size}: $b=c \cdot K  $; 

    \While{$|\hat\gD| < K$}{
        {Compute Matching Score for each $z$:} 
        $m_{\vz} = \text{matching}(\vz, \dval)$ using \eqref{eq:match};
        
        {Select a subset of $b$ datapoints with top-k $m_z$ scores:} $\dfull' = \arg\max_b \{m_z; \forall z \in \mathcal{D}\}$

        {Select a random subset of selected examples:} $\hat\gD = \mathrm{RandomSample} (\dsub, q)$

        {Compute Diversity Score:}
        $\forall z \in \dfull', d_z = \mathrm{diversity}(z, \hat\gD)$
        
        {Add the example that maximize diversity:}
        $\vz = \arg\max \{d_z; \forall z \in \mathcal{D}'\}$
        $\dsub = \dsub \cup \{\vz\}$
       
    }
    
    \Return{$\dsub$}
\end{algorithm*}
\fi

==> sections/intro_v2.tex <==
\section{Introduction}
Instruction tuning is key to enhance the capabilities and controllability of large language models (LLMs) to make models follow instructions~\cite{sanh2022multitask,wei2022finetuned,wang2022super, shen2023flan, ouyang2022training, alpaca, touvron2023llama2,zhang2023instruction}. The main focus of instruction tuning so far has been building general-purpose chatbots,  
this has driven a surge of interest in the creation of instruction-tuning and chat-based datasets~\cite{xu2023baize,xu2023wizardlm,mukherjee2023orca,DatabricksBlog2023DollyV2,kopf2023openassistant,zhou2023lima, ding2023enhancing}. 




Large language models (LLMs) can be rapidly adapted to specific domains and use cases (e.g., question answering) through instruction tuning.
Given the scarcity of in-domain data for these tasks, instruction tuning often requires the model to learn this capability from general data.
However, recent works have suggested that performing instruction tuning with large, aggregated datasets can harm the development of individual capabilities in the model.
This prompts a crucial question:
\begin{center}\emph{Given just a few downstream task examples, how can we effectively select relevant instruction tuning data from a large available pool?}\end{center}



We call this setting \emph{targeted instruction-tuning}.
Prior works on dataset selection have used model representations and $n$-gram features to find datapoints that can improve performance on a target validation set.
Despite their intuitive appeal, it is difficult to rigorously understand how training on these selected datasets will affect the development of a target capability in the LLM.
We instead take inspiration from influence functions to select datapoints that, when trained on, will minimize the loss on a target validation task.
Our algorithm, dubbed \ours{}, exhibits the following desirable properties:

\begin{enumerate}
	\item \textbf{Optimizer-Aware}: \ours{} adapts classical first-order influence functions to operate with the Adam optimizer.
	\item \textbf{Efficient}: \ours{} uses LoRA and random projections to construct low-dimensional gradient features that are time- and memory-efficient while preserving crucial properties for effective dataset selection.
	\item \textbf{Transferable}: We find that data selected using smaller models induces strong performance in larger models as well. Moreover, the design of \ours{} enables efficient and effective dataset selection for new, previously unseen validation tasks.
\end{enumerate}

Experiments on three diverse downstream tasks demonstrate that \ours{} selects data subsets that match or outperform training on the full dataset despite containing significantly fewer examples and having access to only a few validation task examples.
\ours{} also outperforms existing baselines for data selection.
\sm{Mengzhou, fill this in}









==> sections/introduction.tex <==


\section{Introduction}


% general instruction tuning.
Large language models (LLMs) provide a strong foundation for performing various natural language tasks. LLM capabilities can be rapidly improved through instruction tuning, which enables them to follow natural language instructions~\cite{sanh2022multitask,wei2022finetuned,wang2022super, shen2023flan, ouyang2022training, alpaca, touvron2023llama2}. 
This has driven a surge of interest in the creation of instruction-tuning and chat-based datasets~\cite{xu2023baize,xu2023wizardlm,mukherjee2023orca,DatabricksBlog2023DollyV2,kopf2023openassistant,zhou2023lima, ding2023enhancing}. 

The diversity and scale of these datasets, combined with the lack of a clear desired behavior of instruction-tuned models, present unique challenges.
Designing a method to induce strong performance on a targeted downstream application, such as multilingual question answering, is especially difficult. Prior works~\citet{wang2023far} have shown that simply combining instruction tuning data can harm performance on individual downstream tasks. Furthermore, in real-world scenarios, access to in-domain data for the target task is often limited, creating a critical question: 

\begin{center}\emph{Given just a few downstream task examples, how can we effectively select relevant fine-tuning data from a large pool of instruction tuning datasets?}\end{center}

We call this setting \emph{targeted instruction tuning}. Existing approaches to data selection have explored techniques such as domain-specific pre-training~\cite{gururangan2020don} and ngram-based importance resampling~\cite{xie2023data}. However, these methods often rely on token-level features, which may not fully capture the underlying task-specific skills required for effective transfer. Recent work in \citet{han2023understanding} uses gradient information to iteratively select pre-training data to improve in-context learning, but this online approach incurs a large computational expense. 

We address these shortcomings by introducing Gradient-based Data Selection (\ours{}, \textsection\ref{sec:method}), a computationally efficient and effective approach for targeted instruction tuning. \ours{} adapts first-order influence functions for Adam optimizers, and derives the key metric \emph{projected gradient matching} to identify relevant training data for a few validation datapoints. Additionally, \ours{} incorporates a diversity objective to encourage selecting a non-redundant training dataset. Specifically, our algorithm exhibits the following desirable properties:

\begin{enumerate}
    \item \textbf{Computationally efficient (\textsection\ref{sec:method}, \textsection\ref{subsec:efficiency}): } \ours{} derives a first order gradient-based influence function for Adam optimizers. Compared to \citet{han2023understanding}, \ours{} uses LoRA gradients and random projection to construct low-dimensional gradient features that we can efficiently operate on. Moreover, the algorithm allows for efficient reuse of stored gradient features across different downstream tasks.
    \item \textbf{Broadly effective  (\textsection\ref{subsec:main}): } Experiments on three diverse downstream tasks, \mmlu{}, \tydiqa{}, and \bbh{}, demonstrate that \ours{} matches or outperforms training on the entire dataset, despite using very few examples for data selection. Our approach consistently outperforms existing data selection methods.
    \item \textbf{Transferable across model scales (\textsection\ref{subsec:main}):} Data selected using smaller models (e.g., \llamasmall), induce strong performance when tuning larger models (e.g., \llamalarge). For example, training a large model using only $5\%$ of the available data, chosen by a smaller model, can outperform training the large model on the entire dataset. \ours{} is thus amenable to operating on larger models.
    \item \textbf{Interpretable (\textsection\ref{subsec:qualitative}): } Qualitative analysis shows that \ours{} selects data with similar reasoning and skill types as the target task, whereas existing approaches often select data based on surface form cues (e.g., language or topic).
\end{enumerate}




==> sections/method.tex <==
%!TEX root = ../main.tex

\section{Our approach: \ours{}}
\mz{confusing titles, and make people feel that section 2 and 3 are both our contributions
mention the two challenges - propose using influence functions for data selection ()new
challenges
- optimization aware
- efficiency  
}
\label{sec:method}
Our goal is to select a subset $\dsub$ of a large, diverse instruction tuning dataset $\dfull$ such that training a model on $\dsub$ achieves superior performance on a target validation dataset $\dval$, and therefore performs well on the test data.  
Below, we describe how we can efficiently compute the gradient features for both training and validation examples using LoRA~\citep{hu2021lora} and random projections~\citep{Johnson1984ExtensionsOL, park2023trak}.
Then, we detail how our data selection algorithm uses these features. 

\subsection{Notation}
We follow the standard autoregressive setting for instruction tuning, where a datapoint $\vz$ consists of an instruction $\vi$ and a completion $\vc$.\footnote{Some datasets contain multi-turn instructions, but we denote them as single-turn instructions for ease of exposition.} 
For each data point, the loss $\ell(\vz;\vtheta)$ is computed as the cross entropy between the model output $f(\vc\vert\vi)$ and the true label $\vc$.\footnote{When $\vc$ contains multiple tokens, we use an average of the token-wise cross-entropies as the loss for the example.} We use $\vtheta^t$ to indicate the model at the $t$-th step, and we use $\vtheta_i$ to indicate the model after the $i$th epoch of training.
$\dval$ can contain several subtasks $\valsub{1}, ..., \valsub{m}$ (e.g., question answering for multiple languages).\footnote{This is case for datasets we study in this paper, but we note that our method can still apply to datasets with no explicit substructures (i.e., $m=1$)}


\subsection{Efficient Gradient Feature Computation}
\label{sec:grad_features}
Computing \Cref{def:influence} requires taking the inner product of two vectors with as many coordinates as there are trainable parameters in the model.
Directly using such high-dimensional gradient vectors as features for dataset selection is very computationally expensive, so we apply two techniques to construct meaningful low-dimensional gradient features: parameter efficient fine-tuning via LoRA~\citep{hu2021lora} and random projections~\citep{Johnson1984ExtensionsOL, park2023trak}.
We apply these techniques to $\grad{\vz'}{\vtheta}$ for validation datapoints $\vz'$ and to $\update{\vz}{\vtheta}$ for training datapoints $\vz$.
To enable rapid transfer to new target validation tasks, we create a datastore with these low-dimensional features for training datapoints.

\paragraph{Step 1: Warmup training with LoRA.}
% The influence function derived in~\Cref{subsec:adam_inf} requires taking the inner product of two vectors with the same dimensionality as the trainable parameters in the model. 
We use LoRA~\citep{hu2021lora} to reduce the number of trainable parameters and accelerate the inner products in~\Cref{def:influence}.
LoRA freezes the pre-trained weights and adds a low-rank adaptor to fully-connected layers throughout the network.
We use LoRA to instruction tune a pre-trained base model (e.g., \llamasmall{}) on a random subset $\mathcal{D}_\mathrm{warmup} \subset \gD$ for $N$ epochs, checkpointing the model after each epoch to store $\{\vtheta_i\}_{i=1}^N$.
The gradient when training with LoRA, denoted $\loragrad{\cdot}{\vtheta}$, is much lower dimensional than the model itself; for example,  in \llamasmall{}, $\loragrad{\cdot}{\vtheta}$ is less than $2\%$ the size of $\vtheta$.
We use $\loragrad{\cdot}{\vtheta}$ to compute the Adam update and denote it as $\loraupdate{\cdot}{\vtheta}$. We find that this initial warmup training is essential for effective data selection, as relying solely on pre-trained model's gradients for data selection yields suboptimal results (\textsection \ref{subsec:efficiency}). 


\paragraph{Step 2: Projecting the gradients.}
To further reduce the feature dimensionality, we also apply a random projection to the LoRA gradients. %\suchin{we should motivate this over using PCA or something else}
The Johnson-Lindenstrauss Lemma~\citep{Johnson1984ExtensionsOL} asserts that such projections will often preserve the inner products in~\Cref{def:influence}, thereby ensuring these low-dimensional gradient features are still useful for dataset selection. 
For a given validation datapoint $\vz'$ and model checkpoint $\vtheta_i$, we can compute a $\dim$-dimensional projection of the LoRA gradient $\projgrad{\vz'}{\vtheta_i} = \Pi^\top \loragrad{\vz'}{\vtheta_i}$, with each entry of $\Pi\in\sR^{P\times\dim}$ drawn from a Rademacher distribution (i.e., $\Pi_{ij}\sim\gU(\{-1,1\})$). 
For training datapoints $\vz$, we compute $\approxupdate{\vz}{\cdot} = \Pi^\top\loraupdate{\vz}{\cdot}$.  

We use the memory-efficient online implementation of random projections from~\citet{park2023trak} to compute and apply $\Pi$.
In practice, we choose $\dim=8192$ and also normalize the gradient features to ensure that the dot product is equal to the cosine similarity. 
This makes the next step of the procedure much more efficient.

\citet{han2023understanding} is a recent work that uses the gradient information to select supportive pre-training data for in-context learning. We differ from them that we effectively reduce the dimensionality of the gradient features by using LoRA and random projections, and save the features as a gradient store for efficient data selection for multiple downstream tasks.



\iffalse
\paragraph{Learning Rate Schedule.}
The influence function derived above also requires knowing the learning rate used when training on a batch containing $\vz$, denoted as $\eta_t$ in the formula. 
However, $\eta_t$ can change drastically over an epoch, thereby skewing the influences based on the order in which the examples are selected.
To mitigate this issue, we use the average learning rate in each epoch when computing the influence function.
We also treat $1-\beta_1^t\approx 1-\beta_2^t\approx 1$, which is generally the case after a few steps of training.




\subsection{Gradient Feature Computation}\label{sec:grad_features}
As shown above, computing the influence function requires taking the inner product of two vectors with as many coordinates as there are parameters in the model.
Directly using the high-dimensional model gradient vectors as features for dataset selection is computationally expensive, so we apply two techniques to construct meaningful low-dimensional gradient features: parameter efficient finetuning and random projections.
We apply these techniques to $\grad{\vz'}{\vtheta}$ for validation datapoints $\vz'$ and to $\update{\vz}{\vtheta}$ for training datapoints $\vz$.

\paragraph{Training with LoRA}
We use LoRA~\citep{hu2021lora} to instruction tune a pre-trained base model (e.g., \llamasmall{}) on $\gD$ for $N$ epochs, checkpointing the model after each epoch to store $\{\vtheta_i\}_{i=1}^N$.
LoRA is a parameter-efficient tuning method that freezes the pre-trained weights and adds a low-rank adaptor to fully-connected layers throughout the network.
As a result, the gradient when training with LoRA, denoted $\grad{\cdot}{\vtheta}$, is much lower dimensional than the model itself; for example,  in \llamasmall{}, $\grad{\cdot}{\vtheta}$ is less than $2\%$ the size of $\vtheta$.
Note that we use the LoRA gradient for the validation set points and compute $\Gamma$ using the LoRA gradient for points in the training set.

\paragraph{Projecting the Gradients}
To further reduce the gradient dimensionality, we also use a random projection of the gradients. 
It is well-known through the Johnson-Lindenstrauss Lemma that such projections preserve inner products as long as $d$ is large enough, so the projected vectors are meaningful quantities when computing our cosine similarity metric. 
For a given validation datapoint $\vz'$ and model checkpoint $\vtheta_i$, we can compute a $\dim$-dimensional projection of the LoRA gradient $\projgrad{\vz'}{\vtheta_i} = \Pi^\top \grad{\vz'}{\vtheta_i}$, with each entry of $\Pi\in\sR^{P\times\dim}$ drawn from a Rademacher distribution (i.e., $\Pi_{ij}\sim\gU(\{-1,1\})$). For training datapoints $\vz$, we compute $\approxupdate{\vz}{\cdot} = \Pi^\top\update{\vz}{\cdot}$.  

We use the memory-efficient online implementation of random projections from~\citet{park2023trak} to compute and apply $\Pi$.
In practice, we choose $\dim=8192$ to substantially reduce the computation time required to compute the similarity and diversity scores. 
\fi 


\subsection{Step 3: Data Selection Algorithm}\label{subsec:data_select}
The data selection strategy adapts the approach in~\Cref{sec:derivation} to efficiently operate on subtasks of the validation set (e.g., individual tasks within BigBench).
For each subtask $\valsub{i}$, we compute its average gradient feature for every model checkpoint $\vtheta_1,...,\vtheta_N$.
\begin{equation*}
	\avggrad{\valsub{j};\vtheta_i} = \frac{1}{|\valsub{j}|}\sum_{\vz\in\valsub{j}} \projgrad{\vz}{\vtheta_i}
\end{equation*}
As described in~\Cref{def:influence}, we then aggregate the scores of how close the given datapoint is to each validation subtask throughout training.
For example, with Adam, we can write
\begin{equation}
	\infadam(\vz, \valsub{j}) = \sum_{i=1}^N \bar\eta_i \langle \avggrad{\valsub{j}; \vtheta_i}, \approxupdate{\vz}{\vtheta_i} \rangle \label{eq:matching}	
\end{equation}
Finally, we follow the motivation of~\Cref{sec:derivation} to calculate the gradient matching score for $\vz$ as the maximum across all subtasks.
\begin{equation}
	\match{\vz}{\dval} = \max_j \infadam(\vz, \valsub{j})
 \label{eq:match}
\end{equation}
We select the examples with the highest gradient matching score for our experiments. \footnote{We ablate against the analogous form of the algorithm using $\infsgd$ (\Cref{def:influence}) for data selection. See \Cref{app:adam_sgd}.}

\iffalse
\paragraph{Candidate Diversity}
The matching score in \eqref{eq:match} can be viewed as assigning candidate datapoints to validation subtasks (i.e., clusters).
However, given a very large candidate dataset $\dfull$, it is possible that using the matching score alone results in selecting redundant checkpoints.
Thus, we consider a diversity criterion:
\begin{equation*}
	\gK(\vz, \dsub) = -\match{\vz}{\dsub}
\end{equation*}

\paragraph{Selection Algorithm}
Our method is outlined in~\Cref{alg:subset}.
First, we measure the matching score in~\eqref{eq:match} for every datapoint $\vz\in\dfull$.
Then, iteratively, we select the datapoint with the highest diversity score among the $\lfloor cK\rfloor$ candidates with the highest matching scores, where $c$ is a hyperparameter and $K$ is the desired subset size. The selection process prioritizes the data point that contributes the most diversity to the existing set among these top-matching candidates.
\fi

\iffalse
\subsection{Efficient Transferability}
Instead of recomputing gradients for every new target validation task~\citep{han2023understanding}, we store the gradient features for all $\vz\in\dfull$.
Then, when a new validation task $\dval'$ arrives, we can quickly apply our data selection algorithm to identify a good training set.





\subsection{Gradient-based Data Selection}
\paragraph{Step 1: Initial training With LoRA}
We use LoRA~\citep{hu2021lora} to instruction tune a pre-trained base model (e.g., \llamasmall{}) on $\gD$ for $N$ epochs.
LoRA is a parameter-efficient tuning method that freezes the pre-trained weights and adds a low-rank adaptor to fully-connected layers throughout the network.
As a result, the gradient when training with LoRA $\grad{\cdot}{\vtheta}$ is much lower dimensional than the model itself; for example,  in \llamasmall{}, $\grad{\cdot}{\vtheta}$ has less than $2\%$ as many coordinates as $\vtheta$.
%($1.95\%$) 
We save the model parameters at the end of each epoch, denoted as $\vtheta_i$ for the $i$th epoch.


\paragraph{Step 2: Computing projected gradients}
For a given datapoint $\vz$ and model checkpoint $\vtheta_i$, we can compute a $\dim$-dimensional projection of the LoRA gradient $\projgrad{\vz}{\vtheta_i} = \Pi^\top\grad{\vz}{\vtheta_i}$, with each entry of $\Pi\in\sR^{P\times\dim}$ drawn from a Rademacher distribution (i.e., $\Pi_{ij}\sim\gU(\{-1,1\})$).
We use the memory-efficient online implementation of random projections from~\citet{park2023trak} to compute and apply $\Pi$.
In practice, for $P=XXX$ \sm{Mengzhou, fill in} we choose $\dim=8192$ to substantially reduce the computation time required to compute the similarity and diversity scores. \mz{Need to expand z to instruction and completions}


\paragraph{Step 3: Gradient Matching} 
We score how similar a given candidate datapoint $\vz\in\dfull$ is to the target dataset $\dval$. 
We use the cosine similarity of the projected gradients as a proxy for the similarity of two datapoints $\vz$ and $\vz'$. 
Then, the matching score of $\vz$ and the target dataset $\dval$ at checkpoint $i$ is computed as the average pointwise similarity:
$$ \text{sim} (\vz, \dval, i) = \frac{1}{|\dval|}\sum_{\vz'\in\dval} \text{sim} (\vz, \vz', i)$$
where
$$
\text{sim} (\vz, \vz', i) = \cos(\projgrad{\vz}{\vtheta_i}, \projgrad{\vz'}{\vtheta_i})
$$
Finally, we aggregate the similarity score across all of the model checkpoints $\vtheta_1,...,\vtheta_N$ to compute the matching score:
\begin{equation}
	\match{\vz}{\dval} = \frac 1N \sum_{i=1}^{N}\bar\eta_i \cdot \text{sim}(\vz, \dval, i)
	\label{eq:match}
\end{equation}
where $\bar\eta_i$ is the average learning rate used during the $i$th epoch.
This formula is closely related to standard notions of influence~\citep{pruthi2020estimating} when the training dynamics can be approximated by the first order Taylor expansion~\citep{malladi2023kernel}. 
We discuss these connections and how they interact with the Adam optimizer in detail in the appendix.

Some target datasets, such as Big Bench Hard (BBH)~\citep{suzgun2023challenging}, contain multiple tasks $\dval^{(1)},...,\dval^{(m)}$.
Then, we compute the matching score for $\vz$ as the maximum similarity across all of these tasks: 
$\match{\vz}{\dval} = \max_j \match{\vz}{\dval^{(j)})}$.
This procedure ensures better coverage of subclusters within the validation set.

\paragraph{Step 4: Gradient diversity} 
Selecting all examples of $\dsub$ using the matching score risks the inclusion of redundant examples at the cost of good coverage over the original data distribution $\dfull$. 
Thus, we add a diversity criterion that checks if $\vz$ is dissimilar to the examples already selected $\hat\gD\subseteq\dsub$ for training:
\begin{equation}
	\diverse{\vz}{\hat\gD} = -\match{\vz}{\hat\gD}
	\label{eq:div}
\end{equation}

\paragraph{Step 5: Construct $\dsub$} 
The algorithm is outlined in \Cref{alg:subset}.
Given the projected gradients $\{\projgrad{\vz}{\vtheta_i}\}_{i=1}^N$ for every example $\vz\in\gD$, we construct $\dsub$ by finding examples that maximize the matching score in~\eqref{eq:match} and the diversity score in~\eqref{eq:div}.
First, we compute the matching score for every candidate example $\vz\in\gD$ and initialize the selected subset $\dsub$ with the example that has the highest matching score.
Then, we repeat the following procedure until $\dsub$ is full. First, take a set of candidate examples that have the highest matching score. Then, select the candidate that has the highest diversity score against a subsample of the selected dataset.
We ensure that $\dsub$ has no repeated examples.

\fi


==> tables/dimensions.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lccccc} \toprule
    25\%    & \multicolumn{1}{l}{random} & 1024 & 2048 & 4096                 & 8192          \\ \midrule
    MMLU    & \textbf{48.2}              & 50.2 & 51.0 & 51.5                 & \textbf{51.2} \\
    BBH     & \textbf{40.8}              & 42.3 & 43.3 & 42.4                 & 43.2          \\
    TydiQA  & \textbf{53.2}              & 54.6 & 57.6 &                      & \textbf{58.5} \\
    average & 47.4                       & 49.0 & 50.7 & 46.9                 & 51.0        \\ \bottomrule 
    \end{tabular}
    \caption{Results of different gradient projection dimensions when selecting $25\%$ of data from the training set. Even though we reduce the projection gradients to $1024$ dimensions, \simdiv{} still outperforms random selection.}
    \label{tab:dimensions}
\end{table}

==> tables/large_model.tex <==
% \begin{table}[t]
%     \setlength{\tabcolsep}{2pt}
%     \centering
%     \begin{tabular}{@{}cccccc@{}}
%     \toprule
%     & & \multicolumn{4}{c}{\textbf{\llamalarge}} \\
%     \cmidrule(lr){3-6}
%           &  & \textbf{Rand.}      & \textbf{LoRA-7B} & \textbf{LoRA-13B} & \textbf{Full}  \\ \midrule
%     \multirow{2}{*}{\textbf{MMLU}} & $5\%$                          & 53.9                 & \textbf{56.0}           & \textbf{56.0}  &   \multirow{2}{*}{54.7} \\
%                                    & $25\%$                          & 54.4                 & 54.8                    & \textbf{55.5}            \\ 
%                                 \midrule 

%     \multirow{2}{*}{\textbf{TydiQA}}        & $5\%$                          & 51.9                 & 57.1                    & \textbf{60.4} &  \multirow{2}{*}{54.8} \\ 
%                                    & $25\%$                          & 55.4                 & \textbf{59.3}                    & 58.3            \\
%                                    \midrule 

%     \multirow{2}{*}{\textbf{BBH}}           & $5\%$                          & 47.2                 & \textbf{47.5}                    & 45.2   &    \multirow{2}{*}{48.0} \\ 
%                                    & $25\%$                          & 48.2                 & \textbf{48.9}           & 48.1            \\
%                                     \bottomrule
%                                 %    & Full                          & & {48.0}          &                                \\ \bottomrule
%     \end{tabular}
%     \caption{Results of training \llamalarge{} on data selected by a small model (LoRA-7B) and a larger model  (LoRA-13B) using \ours{}. With merely $5\%-25\%$ data, the performance of the large model outperforms the full dataset. This suggests that we can use a small model to select data for a larger model.}
%     \label{tab:largemodel}
    
% \end{table}



\begin{figure*}[t]
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/llama-13b.pdf}
        \caption{Training \llamalarge{} on selected data.}
        \label{fig:training_percentage}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mistral.pdf}
        \caption{Training \mistral{} on selected data.}    
        \label{fig:projected_dimension}    
    \end{subfigure}
    \caption{Training \llamalarge{} and \mistral{} with $5\%$ data selected by LoRA-7B outperforms not only random selection, but also training with the full dataset. \ours{} by LoRA-7B denotes that the data is selected with the gradients from LoRA-7B. \ours{} denotes that the data is selected with the gradients of the target LoRA model. }
\end{figure*}

==> tables/lorap.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lcccc} \toprule
    25\%    & random        & \textbf{0.25} & \textbf{0.5} & \textbf{1}    \\ \midrule
    MMLU    & 48.2 & 50.7         & \textbf{51.9}        & 51.2 \\
    BBH     & 40.8 & 42.4         & 42.4        & 43.2          \\
    TydiQA  & 53.2 & 57.6         & 56.8        & 58.5 \\
    average & 47.4          & 50.2         & 50.4        & 51.0        \\ \bottomrule 
    \end{tabular}
    \caption{Training the initial model with $25\%$, $50\%$ and $100\%$ of the data. Training with $25\%$ of the data is sufficient to lead to siginificant improvemet over random selection.}
    \label{tab:lorap}
\end{table}

==> tables/rep_grad.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{lcccc} \toprule
    & \textbf{Random} & \textbf{Rep} & \textbf{Grad} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-4}
    \mmlu & 46.7 & 45.9 & 51.1 \\
    \tydiqa & 50.7 & 51.6 & 55.7 \\
    \bbh & 38.2 & 39.4 & 39.7 \\ \midrule
    Avg. & 45.2 & 45.7 & \textbf{48.8} \\ \bottomrule
    \end{tabular}}
\caption{Performance of using the representations (Rep) and projected gradients (Grad) for data selection (w/o using the diversity term). We select $5\%$ of the data for instruction tuning.}
\label{tab:rep_grad}
\end{table}
    
    

==> tables/simdiv.tex <==
    \begin{table}[t]
        \centering
        \begin{tabular}{lrcc} \toprule
                       &      \textbf{\% Data}        & \textbf{\ours{} w/o div} & \textbf{\ours} \\ \midrule
        \multirow{2}{*}{\textbf{MMLU}}   & 5\%                 & 51.1          & 51.1        \\
                                         & 10\%                          & 50.2          & 50.9  \ua{0.7}        \\ 
                                         & 25\% & 51.7 & 51.7 \\
                                         & 50\% & 52.5 & 51.8 \da{0.7} \\ 
                                         \midrule
                                         \multirow{2}{*}{\textbf{TydiQA}}    & 5\%                          & 55.7          & 56.5     \ua{0.8}     \\
                                         & 10\%                          & 56.2          & 56.8   \ua{0.6}       \\ 
                                         & 25\% & 56.5 & 55.6 \da{0.9} \\
                                         & 50\% & 53.0 & 55.9 \ua{2.9} \\ \midrule 
        \multirow{2}{*}{\textbf{BBH}} & 5\%                          & 39.7         & 41.3    \ua{1.6}      \\
                                         & 10\%                          & 40.8          & 41.9  \ua{1.1}      \\ 
                                         & 25\%                          & 43.1          & 42.2  \da{0.9}      \\ & 50\%                          & 41.4          & 42.6  \ua{1.2}      \\  
                                         \bottomrule 
        \end{tabular}
        \caption{Ablations on \ours{} without the diversity term. Adding a diversity term mostly helps especially in a small dataset size, but is less useful or even hurts when the dataset size increases.}
        \label{tab:div}
    \end{table}
    

==> tables/source_model_p0.25.tex <==
\begin{table*}[t]
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{tabular}{lccccccccc} \toprule
        & &  \multicolumn{4}{c}{\textbf{Pre-trained Models}} & \multicolumn{4}{c}{\textbf{LoRA Models}} \\
           & \textbf{Random} & \multicolumn{2}{c}{\textbf{Llama2-7B}} & \multicolumn{2}{c}{\textbf{Llama2-7B-chat}} & \multicolumn{2}{c}{\textbf{Second Checkpoint}} & \multicolumn{2}{c}{\textbf{Multi. Checkpoints}} \\ \cmidrule(lr){1-1} \cmidrule(lr){2-2}  \cmidrule(lr){3-6} \cmidrule(lr){7-10}
           &  & Rep          & Grad         & Rep            & Grad            & Rep                  & Grad                  & Rep                   & Grad                 \\ 
           \cmidrule(lr){1-1} \cmidrule(lr){2-2}  \cmidrule(lr){3-6} \cmidrule(lr){7-10}
    \mmlu & 48.2 & 50.0          & 49.1          & 47.0            & 47.9             & 49.5                  & 50.3                   & 48.7                   & \textbf{51.7}         \\
    \tydiqa & 52.5 & 51.0          & 52.9          & 53.4            & 55.1             & 54.1                  & 55.9 & 55.8                   & \textbf{56.5}         \\
    \bbh  & 38.8  & 41.4          & 43.2          & 41.9            & 41.3             & 41.5                  & 41.2                   & \textbf{43.4}          & 43.1     \\     \midrule
    Avg. & 46.5 & 47.5 & 48.4 & 47.4 & 48.1 & 48.4 & 49.2 & 49.3 & 50.4
    \\ \bottomrule       
    \end{tabular}}
    \caption{Performance of using the representations (Rep) and projected gradients(Grad) from different source models for data selection. Note that the diversity term is excluded for purely comparing the effect of approaches for data representations. We select $25\%$ of the data for instruction tuning. }
    \label{tab:rep_grad}
\end{table*}

==> tables/trainp.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.98\columnwidth}{!}{%
    \begin{tabular}{lcccc}
    \toprule
                     & \multicolumn{1}{l}{\textbf{}} & \multicolumn{3}{c}{\textbf{\# Data for LoRA Training}} \\  \cmidrule(lr){3-5} 
    \textbf{}        & \textbf{Random}               & \textbf{65K (25\%)}    & \textbf{130K (50\%)}     & \textbf{260K (100\%)}     \\ \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5}
    \textbf{MMLU}    & 46.7                          & 50.7             & 50.2             & \textbf{51.1}    \\
    \textbf{TydiQA}  & 50.7                          & \textbf{57.7}    & 56.4             & 56.6             \\
    \textbf{BBH}     & 38.2                          & 41.1             & \textbf{41.5}    & 41.3             \\ \midrule
    \textbf{Average} & 45.2                          & \textbf{49.8}    & 49.4             & 49.7         \\ \bottomrule  
    \end{tabular}}
    \caption{Performance of using different number of data for LoRA training. We find that using $25\%$ data for training the LoRA model is sufficient for data selection on average.}
\end{table}

==> tables/zero_shot.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.4\columnwidth}{!}{%
    \begin{tabular}{@{}lcccc@{}}
    \toprule
                    & \multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{Fine-tuning Llama2-7b with}}           \\
                    \cmidrule(lr){3-5}
                    & \textbf{Llama2-7b}   & \textbf{Valid.} & \textbf{Rand. 5\%} & \textbf{\ours 5\%} \\
                    \cmidrule(lr){2-2} \cmidrule(lr){3-5}
    \textbf{\mmlu}   & 45.6                 & 47.3                 & 46.7               & 51.3             \\
    \textbf{\tydiqa} & 46.4                 & 52.0                 & 50.7               & 56.4             \\
    \textbf{\bbh}    & 38.3                 & 37.4                 & 38.2               & 40.1             \\ \bottomrule
    \end{tabular}}
    \caption{Performance of \llamasmall{} without fine-tuing, fine-tuning with validation data, and fine-tuning with $5\%$ of randomly selected data and $5\%$ data selected by \ours. Essentially, fine-tuning with validation data outperforms fine-tuning with $5\%$ of randomly selected data, but lags behind \ours{}.}
    \label{tab:zero_shot}
\end{table}
